Noisy Symbolic Abstractions for Deep RL: A case study with Reward Machines

Natural and formal languages provide an effective mechanism for humans to specify instructions and reward functions. We investigate how to generate policies via RL when reward functions are specified in a symbolic language captured by Reward Machines, an increasingly popular automaton-inspired structure. We are interested in the case where the mapping of environment state to a symbolic (here, Reward Machine) vocabulary -- commonly known as the labelling function -- is uncertain from the perspective of the agent. We formulate the problem of policy learning in Reward Machines with noisy symbolic abstractions as a special class of POMDP optimization problem, and investigate several methods to address the problem, building on existing and new techniques, the latter focused on predicting Reward Machine state, rather than on grounding of individual symbols. We analyze these methods and evaluate them experimentally under varying degrees of uncertainty in the correct interpretation of the symbolic vocabulary. We verify the strength of our approach and the limitation of existing methods via an empirical investigation on both illustrative, toy domains and partially observable, deep RL domains.

==> coverpage.tex <==
@article{hill-arxiv2020,
  author    = {Felix Hill and
               Sona Mokra and
               Nathaniel Wong and
               Tim Harley},
  title     = {Human Instruction-Following with Deep Reinforcement Learning via Transfer-Learning
               from Text},
  journal   = {CoRR},
  volume    = {abs/2005.09382},
  year      = {2020}
}

https://arxiv.org/abs/2005.09382




==> figs/flowchart.tex <==
\begin{figure}[h]
  \begin{center}
    \includegraphics[width=0.75\textwidth]{figs/flowchart5.pdf}
  \end{center}
  \caption{In the reward machine framework, high-level propositions $\mathcal{AP}$ of the state $s_t$ are described by a labelling function $\mathcal{L}$, providing a vocabulary for the specification of non-Markovian tasks via reward machines. Our work targets real-world settings where the labelling function $\mathcal{L}$ is not freely available at deployment time or challenging to model perfectly. We raise issues with prior methods that approximate \added{the reward machine state} $u_t$ from uncertain propositional values (\textcolor{red}{\textcircled{\small{1}}}) in a task-agnostic manner, and we propose to instead model the task-relevant dynamics of the reward machine (\textcolor{blue}{\textcircled{\small{2}}}).
  \alt{
  In the reward machine framework, high-level propositions $\mathcal{AP}$ of the state $s_t$ are described by a labelling function $\mathcal{L}$, providing a vocabulary for the specification of non-Markovian tasks via a reward machine (RM). Our work targets real-world settings where the labelling function $\mathcal{L}$ is not freely available at deployment time or challenging to model perfectly. We raise issues with prior methods (\textcolor{red}{\textcircled{\small{1}}}) that approximate the reward machine state $u_t$ in a task-agnostic manner using an estimate of the labelling function, and we propose to instead directly estimate the reward machine state (\textcolor{blue}{\textcircled{\small{2}}}).
  }
  }

\commentzc{Maybe we can cross out $\mathcal{L}$ box to show that the perfect labelling function is not available.}
\commentzc{\href{https://docs.google.com/drawings/d/1nrYsJYu0IsF4ly1V8dDMgP_Dq45oz1nqSWIGB4drQoY/edit}{editable link}}


==> sections/abstract-long.tex <==
\begin{abstract}
Natural and formal languages, including programming languages, provide an effective mechanism for humans to specify reward functions, task specifications, and instructions to Reinforcement Learning (RL) agents. However, RL agents need to be able to relate their depiction of environment state\remove{, be it as pixels or other perceptual input,} to the symbolic vocabulary and sentences of those languages. In this paper we examine how to generate policies via RL when reward functions are specified via a formal language and expressed in an increasingly popular automaton-inspired structure called a Reward Machine. We are interested in the case where the mapping of environment state to the symbolic vocabulary used to describe the reward function is noisy. We formulate the problem of policy learning in Reward Machines with noisy symbolic abstractions as a special class of POMDP optimization problem, and investigate several methods to address the problem building on existing and new techniques %proposed in here.
\remove{the latter focused on predicting Reward Machine state, rather than on grounding of individual symbols.} We analyze these methods and evaluate them experimentally under varying degrees of uncertainty in the correct interpretation of the symbolic vocabulary.
%
We verify the strength of our approach and the limitation of existing methods via an empirical investigation on both illustrative, toy domains and partially observable, deep RL domains.
\end{abstract}


==> sections/old-theorems.tex <==

\section{Additional Definitions, Theorems, and Proofs}

\begin{definition}[\emph{Cross Product Belief MDP}]
\label{def:cross_product_belief_mdp}
Given a URM-MDP $\mathcal{K}$ associated with RM-MDP \revisit{$\langle S, T, A, P, \gamma, \mu, U, u_0, F, \mathcal{AP}, \delta_t, \delta_r, \mathcal{L} \rangle$}, we define a cross product belief MDP as an MDP $\mathcal{K}_U$ with state space $S' = S \times \tilde{U}$ (where $\tilde{U}$ are the set of beliefs over $U$, i.e. $|U|$-dimensional probability vectors), action space $A' = A$, and discount factor $\gamma'=\gamma$. 

Now we define the transition probabilities, initial state distribution, and reward function for the cross product belief MDP. To simplify notation, define $b_u: (S \times A)^* \times S \rightarrow \tilde{U}$, $b_u(s_0, a_0, \ldots, s_{t-1}, a_{t-1}, s_t) = \pr(\cdot | s_0, a_0, \ldots, s_{t-1}, a_{t-1}, s_t)$ to be the Bayesian belief of the unknown RM state $u_t$ given the state-action history. 

Then, the transition probabilities are $P'(s_{t+1}, \tilde{u}_{t+1} | s_t, \tilde{u}_t, a_t) = P(s_{t+1} | s_t, a_t) \cdot \mathbb{I}[\tilde{u}_{t+1} = b_u(s_0, a_0, \ldots, s_t, a_t, s_{t+1})]$, the initial state distribution is $\mu'(s_0, \tilde{u}_0) = \mu(s_0) \mathbb{I}[\tilde{u}_0 = b_u(s_0)]$, and the (stochastic) reward function is given by $R'(r_t | s_t, \tilde{u}_t, a_t, s_{t+1}, \tilde{u}_{t+1}) = \sum_{u_t \in U} {p(u_t | \tilde{u}_t) \delta_r(u_t, \mathcal{L}(s_t, a_t, s_{t+1}))}$. 

\end{definition}

\bigskip 
\begin{theorem}[Optimal Policy in a URM-MDP]
\label{theorem:rm_belief}
Given a URM-MDP $\mathcal{K}$ associated with RM-MDP \revisit{$\langle S, T, A, P, \gamma, \mu, U, u_0, F, \mathcal{AP}, \delta_t, \delta_r, \mathcal{L} \rangle$}, there exists an optimal policy of the form $\pi(a | s, \tilde{u})$, where $a \in A, s \in S$ and $\tilde{u}$ is the belief distribution over reward machines states $U$ given the history of states and actions, i.e. $\tilde{u}(u) = \pr(u_t = u | s_0,a_0, \ldots, s_{t-1}, a_{t-1}, s_t)$.

\medskip
\emph{Proof.} It is well known that any POMDP can be formulated as an equivalent \emph{belief MDP} whose states are beliefs over the original states of the POMDP (\cite{aastrom1965optimal}). In the case of a URM-MDP $\mathcal{K}$, the corresponding belief MDP $\mathcal{K}_{S \times U}$ (whose states are beliefs over $S \times U$) is equivalent to the cross product belief MDP $K_{U}$, in the following sense. A state at time $t$ in the belief MDP $K_{S \times U}$ is a distribution $b_t$ over $S \times U$. However, in a URM-MDP, $s_t \in S$ is known and observable at time $t$, thus the distribution $b_t$ must only assign positive probability to states $(s,u) \in S \times U$ where $s = s_t$. $b_t$ can equivalently be represented as $(s_t, \tilde{u})$, where $\tilde{u}$ is the belief distribution over $U$. The transitions in the cross product MDP $K_{U}$ precisely mimic those in the belief MDP $K_{S \times U}$, bar this change in representation.

Hence, solving a URM-MDP is equivalent to solving the corresponding cross product belief MDP, which has an optimal solution of the form $\pi^*(a_t | s_t, \tilde{u}_t)$, where $\tilde{u}_t$ is the Bayesian belief over $u_t$, given $s_0, a_0, \ldots, s_{t-1}, a_{t-1}, s$.  
\qed
\end{theorem}

\bigskip
\begin{definition}[\emph{Uncertain-Proposition Reward Machine POMDP} \textbf{(URM-POMDP)}]
\label{urmpomdp}
Given a POMDP (without reward function) $\mathcal{M} = \langle {S},\Omega, {T},{A},{P}, {O}, \gamma, \mu \rangle$, a finite set of atomic propositions $\mathcal{AP}$, a (ground-truth) labelling function $\mathcal{L}: S\times A \times S \rightarrow 2^{\mathcal{AP}}$, and a reward machine $\mathcal{R} = \langle U, u_0, F, \delta_u, \delta_r \rangle$, a {URM-POMDP} is a POMDP $\mathcal{K} = \langle S_\mathcal{K}, \Omega_\mathcal{K}, T_\mathcal{K}, A_\mathcal{K}, P_\mathcal{K}, O_\mathcal{K}, R_\mathcal{K}, \gamma_\mathcal{K}, \mu_\mathcal{K} \rangle $ with state space $S_\mathcal{K} = S \times U$, observation space $\Omega_\mathcal{K} = \Omega$, terminal states $T_\mathcal{K} = (T\times U)\cup (S\times F)$, action space $A_\mathcal{K} = A$, transition probabilities $P_\mathcal{K}((s_{t+1}, u_{t+1}) | (s_t,u_t),a_t) = P(s_{t+1}|s_t,a_t) \cdot \mathbbm{1}[\delta_u(u_t, \mathcal{L}(s_t, a_t, s_{t+1})) = u_{t+1}]$, observation probabilities $O_\mathcal{K}(o_t|(s_t,u_t), a_t) = O(o_t|s_t,a_t)$, reward function $R_\mathcal{K}((s_t,u_t),a_t,(s_{t+1},u_{t+1})) = \delta_r(u_t, \mathcal{L}(s_t, a_t, s_{t+1}))$, discount factor $\gamma_\mathcal{K}=\gamma$ and initial state distribution $\mu_\mathcal{K}(s,u) = \mu(s)\mathbbm{1}[u = u_0]$.
%\commentzc{Similar as above}
\end{definition}

\bigskip
\begin{theorem}[Optimality of \ttt{RMSM}]
\label{theorem:rmsm}
Let $\mathcal{K}$ be a URM-MDP or URM-POMDP, $\pi_\theta$ a policy, and $g_\phi$ an RM state belief predictor as defined in the \ttt{RMSM} algorithm. Assume that every feasible trajectory in $\mathcal{K}$ occurs with non-zero probability under $\pi_\theta$. If $g_\phi$ minimizes $L_\phi$ with respect to $\phi$ and $\pi_\theta$ maximizes $J_\theta$ with respect to $\theta$, then $\pi_\theta$ is an optimal policy in $\mathcal{K}$ and $g_\phi$ matches the ground-truth belief over RM states given the history.

\medskip
\emph{Proof.} First, consider when $\mathcal{K}$ is a URM-MDP. For any particular history $s_0, a_0, \ldots, s_{t-1}, a_{t-1}, s_t$ under $\pi_\theta$, 
$- \log {g_\phi(u_t | s_0, a_0, \ldots, s_{t-1},a_{t-1},s_t)}$ is minimized when $g_\phi(u_t | s_0, a_0, \ldots, s_{t-1},a_{t-1},s_t) = \pr(u_t | s_0, a_0, \ldots, s_{t-1},a_{t-1},s_t)$ from a well-known result about information entropy. Minimizing $L_\phi = \mathbb{E}_{\pi_\theta}[- \log {g_\phi(u_t | s_0, a_0, \ldots, s_{t-1},a_{t-1},s_t)}]$ (with respect to $\phi$) requires that $g_\phi(u_t | s_0, a_0, \ldots, s_{t-1},a_{t-1},s_t) = \pr(u_t | s_0, a_0, \ldots, s_{t-1},a_{t-1},s_t)$ for all feasible histories $s_0, a_0, \ldots, s_{t-1}, a_{t-1}, s_t$, since all feasible histories have positive probability under $\pi_\theta$. In other words, $g_\phi$ matches the ground-truth belief over RM states given the history. 

\medskip
Now consider $\pi_\theta(a_t | s_t, \tilde{u}_t)$, where $\tilde{u}_t = g_\phi(\cdot | s_0, a_0, \ldots, s_{t-1}, a_{t-1}, s_t) = b_u(s_0, a_0, \ldots, s_{t-1}, a_{t-1}, s_t)$, and $b_u$ returns the ground-truth belief over RM states given the history. The inputs $s_t, \tilde{u}_t$ to the policy are precisely the states of the corresponding Cross Product Belief MDP $\mathcal{K}_U$ of $\mathcal{K}$, thus $\pi_\theta$ maximizes the expected discounted return in $\mathcal{K}_U$. This implies $\pi_\theta$ is also an optimal policy in the original URM-MDP $\mathcal{K}$. 
 
 
\medskip
When $\mathcal{K}$ is a URM-POMDP, the proof that $g_\phi$ matches the ground-truth belief over RM states given the history remains virtually unchanged. On the policy side, the \ttt{RMSM} policy is of the form $\pi_\theta(a_t | h_t, \tilde{u}_t)$. Note, however, that there even exists an optimal policy in the URM-POMDP of the form $\pi^*(a_t | h_t)$. Regardless of $g_\phi$, maximizing $J_\theta$ (with respect to $\theta$) can always recover an optimal policy in $\mathcal{M}$ by ignoring $\tilde{u}_t$.
\qed


\end{theorem}


